Devils in the Clouds: An Evolutionary Study of Telnet Bot Loaders

One of the innovations brought by Mirai and its derived malware is the adoption of self-contained loaders for infecting IoT devices and recruiting them in botnets. Functionally decoupled from other botnet components and not embedded in the payload, loaders cannot be analysed using conventional approaches that rely on honeypots for capturing samples. Different approaches are necessary for studying the loaders evolution and defining a genealogy. To address the insufficient knowledge about loaders' lineage in existing studies, in this paper, we propose a semantic-aware method to measure, categorize, and compare different loader servers, with the goal of highlighting their evolution, independent from the payload evolution. Leveraging behavior-based metrics, we cluster the discovered loaders and define eight families to determine the genealogy and draw a homology map. Our study shows that the source code of Mirai is evolving and spawning new botnets with new capabilities, both on the client side and the server side. In turn, shedding light on the infection loaders can help the cybersecurity community to improve detection and prevention tools.

==> parts/v1/00-abstract.tex <==
% !TeX root = ..\main.tex
% Honeypots have always been the sharpest tool to analyze botnets on the Internet, which play an important role in catching the latest bot samples, sensing emerging scans, analyzing state-of-art intrusions, and providing latest vulnerability dynamics. Based on samples captured by honeypots, researchers leverage a bunch of methods to discover the dynamic of botnets to reveal botmasters and variation status. 
Due to the distributed nature of popular botnets, bot authors seldom put all the functions of a botnet in single bot executable.
Self-contained loaders are widely adopted by the botmasters to execute a loading function for spawning new bots, which are commonly running in a cloud environment rather than the edge devices.
Generally, loaders are not loaded on the victim devices, which effectively hinders the researchers from understanding the loaders' implementations using honeypots, and dramactically reduce the feasibility for classifying and tracking.
In this paper, we propose a text-based method to investigate and analyze the bot loader's inner implementation using honeypots.
We regard an interaction log captured by honeypot system as a textual representation of the loader's function, and then cluster all the samples to reveal the similarity between any two loaders.
Based on the clustering results, we push it further to explore the homological relationship among botnets.
Our approach partitions the collected logs to reflect the similarity of loader functions using the natural language processing (NLP) methods.
Differences and similarities between two logs are evaluated to infer homological functions and implementations among two related classes of loaders.
The homology analysis yields a new insight for researchers to identify the botnet's infrastructures and track their evolution over time.
Based on the statistics of our dataset, we discover that the released code of Mirai keeps spawning new generations of botnets not only on the client side but also on the server side. 

\endinput

==> parts/v1/01-intro.tex <==
% !TeX root = ..\main.tex
Accompanying the growth of the IoT market, botnets targeting IoT devices have become a major threat to cyber security.
The IoT botnet is a worm-like malware system targeting monopolizing IoT devices to execute malicious actions.
Nowadays, IoT Botnets have become the most popular solution for attackers conducting DDoS attacks\cite{koliasDDoSIoTMirai2017}, exploiting other hosts\cite{dangUnderstandingFilelessAttacks2019} and even cryptomining\cite{bijmansJustTipIceberg2019}.
Mirai\cite{antonakakisUnderstandingMiraiBotnet2017,malwaremustdie!MMD00562016LinuxMirai2016}, the most famous descendant of classic botnet Bashlite, was recorded launching a 1.1Tbps DDoS attack using 148,000 IoT devices, which broke the record and makes it the top botnet in the following years.
Anna-senpai's code release\cite{anna-senpaiFREEWorldLargest2016} in September 2016 further stimulated botmasters to create variants\cite{herwigMeasurementAnalysisHajime2019} based on its idea.

From the perspective of victim IoT devices, security industries have gathered sufficient intelligence to understand IoT botnets in recent years.
Malware samples collected by honeypots\cite{fanEnablingAnatomicView2018} have been dissected to investigate their functions and analyze their lineage to reach a in-depth yet systematic understanding of botnets' propagation and evolution\cite{dibMultiDimensionalDeepLearning2021,cozziTangledGenealogyIoT2020}.

However, although bot loaders play important roles in exploiting vulnerabilities and injecting bot clients, these server-side components could never be captured by honeypots as they seldom load themselves to victim devices.
Limited methodologies confined recent studies\cite{torabiStringsBasedSimilarityAnalysis2021,tabariWhatAreAttackers2021,lingenfelterAnalyzingVariationIoT2020,antonakakisUnderstandingMiraiBotnet2017,griffioenExaminingMiraiBattle2020,stephensDetectingInternetThings2021} only making simple comparisons on specified properties extracted from interaction logs, yet the infeasibility of dissecting their executable files also impacted the completeness of the server-side perspective of IoT botnets.
The panorama of IoT botnets is still missing the crucial part, which could help security industries inference the backgrounds of cybercrimes from a different aspect.

% 这里不是很好
In this paper, we try to complete the server-side knowledge of botnets by categorizing active bot loaders and mining their homologies at the function level.
To address the absence of captured samples, we treat interaction logs from telnet honeypots as an observation of loaders' workflows and propose an alternative NLP-based methodology to extract crucial information from them.
Our work provides a behavior-based categorization of bot loaders and proposed a new homology view on bot loaders, helping researchers obtain deeper knowledge about IoT botnets.
The main contributions of our work are summarized as follows:

\begin{itemize}
  \item
    Our work provides a server-side perspective for cyber forensics to investigate cybercrimes beside bots.
    %Though we cannot directly access the botnets' infrastructure code or executables, 
    We try to describe loaders' functions using request logs captured by the telnet honeypot, which is an alternative method to understand the inner details of bot loaders.
  \item
    We propose a semantic-aware yet an elastic method for classifying bot loaders based on interaction logs from honeypots.
    We define 8 families out of 19 clusters and describe their behavior similarity based on the result of agglomerative clustering and several empirical criteria.
    We also extracted representative strings for each cluster to show their functional characters, which provides an explainable result for our family definition.
    % Based on the captured request logs, we leverage agglomerative clustering to hierarchically classify active bot loaders into several clusters and apply empirical criteria to refine the family definition.
    % The hierarchical structure of the agglomerative tree reflects the similarity of loaders, which is a solid basis for further homological analysis of their functions.
    % We also extracted representative strings for each cluster to show their functional characters, which provides an explainable result for our family definition.
    % We defined 8 families out of 18 clusters.
    % Despite bot malware may vary frequently, the skeletons of telnet loaders can keep stable across a long period, which demonstrates the widespread adoption of decoupling design in botnets.
  \item 
    We made an in-depth investigation of loaders' behaviors and their relationships.
    To examine the component homologies of loaders, we analyze extracted representative strings associated with the result of agglomerative clustering.
    The common skeleton and shared components across different families are well described based on these results.
    This perspective can provide solid evidence for investigating underground industries to uncover their connections.
    % The investigation on loaders also reveals the diversity of botnets, which could indicate the activity of emerging botnets from the server-side perspective.
    % TODO R2-weakness: The methology chapter did not support the third point mentioned in the main contribution, Please provide more evidence. The original description is as follows: 
    % Yan: Add your results: real interesting observations.
\end{itemize}

\endinput

==> parts/v1/02-backgrounds.tex <==
% !TeX root = ..\main.tex
In the Anna-senpai's release\cite{anna-senpaiFREEWorldLargest2016}, the botnet was designed as a distributed system that consists of 3 major components, \emph{bot}, \emph{loader server}, and \emph{C\&C server}.
The overall architecture is dipicted in Fig. \ref{fig_botnet_arch}.
In the attack phase (\ding{172}), the C\&C server sends attack commands to bots like traditional botnets.
But in the propagate phase, bots only scan for vulnerable devices but never load bot executables (\ding{173}).
They merely report collected IP addresses and credentials to the loader server.
The self-contained loader server executes loading scripts to launch bot malware on victim devices (\ding{174}).
The decoupled loader and distributed architecture simplified its design and robustified its infrastructure to survive taking-downs.


\begin{figure}[tp]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/botnet.pdf}
  \caption{Common botnet architecture.}
  \label{fig_botnet_arch}
  % \Description[<short description>]{<long description>}
\end{figure}

\begin{figure*}[htb]
  \centering
  \includegraphics[width=0.9\textwidth]{figures/methodology.pdf}
  \caption{Schematic depiction of the analysis steps in our work.}
  \label{fig_methodology}
  % \Description[<short description>]{<long description>}
\end{figure*}

To monitor botnets and observe their evolution, researchers continuously gather information and track dynamics to follow up on botnets' entire lifecycle.
Emerging botnets and infected devices are continuously measured to summarize the dynamics of threats.
The first research about Mirai made by Antonakakis et al.\cite{antonakakisUnderstandingMiraiBotnet2017} tried to observe Mirai's spread and evolution from many aspects.
This work utilized a network telescope, scanner, honeypot, DNS probe, and C\&C milker to collect information, then analyzed DDoS records provided by CDN providers.
In this paper, the authors recorded the growth and evolution ever since Mirai first appears, then summarized details about infections, ownerships, and attacks.
By relating C\&C servers, C\&C domain names, and credential dictionaries, this work examined several individual botnets and observed the expansion of their variants.
Many papers \cite{herwigMeasurementAnalysisHajime2019,griffioenExaminingMiraiBattle2020,safaeipourDatadrivenCurationLearning2020} also followed up on the dynamics of botnets and conducted temporal observations of botnet threats.
Wang et al. \cite{wangEvolutionaryStudyIoT2021} applied an NLP-based method to correlate the information published by researchers and constructed a lineage graph for 72 IoT malware families to reflect their evolutionary relationships.

Tracking emerging botnets and their evolution is one of the fundamental tasks for security industries.
While released source codes keep spawning new botnet variants, researchers monitored new samples\cite{paIoTPOTAnalysingRise2015}, new attack vectors\cite{dangUnderstandingFilelessAttacks2019}, and new fingerprints\cite{abbasGenericSignatureDevelopment2021} to measure emerging botnets and relate them with existing ones.
Malware samples of bot clients have been dissected to analyze their function.
Cozzi et al. analyzed the tangled genealogy of botnet malware by comparing samples at the binary level\cite{cozziTangledGenealogyIoT2020}.

As dissecting malware samples is infeasible for bot loaders and related server-side components, researchers tried comparing their intrusion fingerprints to determine the similarities between different loaders.
Numerous papers\cite{lingenfelterAnalyzingVariationIoT2020,torabiStringsBasedSimilarityAnalysis2021,tabariWhatAreAttackers2021,antonakakisUnderstandingMiraiBotnet2017,griffioenExaminingMiraiBattle2020,ghietteFingerprintingToolingUsed2019} compared exploit logs from honeypots to find a lineage of loaders by comparing exploited vulnerabilities, credentials, and intrusion commands.
However, these simple and isolated comparisons are less solid to reach a systematic conclusion on how loaders variated and derived predecessors' codebase.
The security industry is still seeking a new systematic methodology to discover the details of loaders and obtain overall intelligence as we have about those client-side components.

\endinput

==> parts/v1/05-discuss.tex <==
% !TeX root = ..\main.tex
In this paper, we focus on investigating loaders based on the interaction logs.
However, this limited methodology is far from ultimate for mining all covert information of botnets.


\subsubsection*{Associated malware}

Bot client is the most volatile part of botnets, but our work lacks aspects on bot clients.
Combining these two analyses to analyze relationships among loaders and clients may extend the conclusion of homology analysis, which is a feasible and promising field for botnet studies.


\subsubsection*{Family definition}

Our work draws a conclusion based on the result of agglomerative clustering.
The empirical value of \begin{math}\mathcal{T}\end{math} determined the family definition of bot loaders.
However, due to the heterogeneity of loaders' behavior, a homogeneous \begin{math}\mathcal{T}\end{math} cannot fit all situations.
For example, We found that whattttttlol was misclassified along with 6-chars, which reflects our method is still deficient to make a clear definition of classes.
The cutting condition of the agglomerative tree should be further discussed in the following studies.
% Note that the query tokens and credentials are not fully investigated, which could miss critical information of loaders.


\subsubsection*{Early stage detection}

For IDS systems, the loading stage is one of the best chances to intercept emerging attacks.
Our methodology for analyzing network messages push the identification further to recognize the identity of attackers, which is of great importance in reinforcing the security of the Internet.


\endinput

==> parts/v1/06-conclusion.tex <==
% !TeX root = ..\main.tex
% In recent years, the open-source botnets spawned a mass of variants, which is a major threat to IoT devices.
While understanding the behaviors of botnet malware is crucial, their infrastructures, especially loader servers, are not systematically investigated yet.
In this work, we proposed a novel aspect of homology analysis on bot loaders.
We analyze loaders' implementation using honeypot logs and evaluate their relationship by shared components.
Our experiment consists of 3 components.
First, we collect interaction logs using a high interaction honeypot system to represent the functions and behaviors of loader hosts.
Second, we use agglomerative clustering to cluster these logs, fit all relationships onto a tree, and cut at a threshold to classify the loaders.
Finally, we evaluate the tree bottom-top and leverage the align algorithm to evaluate shared components in each loader family.
We find that the ecosystem of Mirai is still active despite numerous takedowns.
New variants are created to satisfy botmasters' needs in many aspects.
We also discover that some small-scale botnets come and fade away in a very short timespan.
%are making an appearance and quickly fading away.
The security community should further develop the methodology of botnet investigation to enhance the knowledge of botnets' relationships, which could help eliminate cybercrimes more efficiently.
%should be more intensively watched to keep the network safe and clean.

\endinput

==> parts/v2-journal/00-abstract-v2.tex <==
% !TeX root = ..\main.tex
% Along with the evolution of IoT botnets, various botnet virology studies have worked on identifying malware families from botnet campaigns and inferring their connections.
% While dissecting malware samples and analyzing their run-time behaviors can provide solid evidence to depict the genealogy of botnet families, their compromising toolkits deployed on loader servers are not yet thoroughly examined due to the infeasibility of capturing their samples.
% Moreover, as these infection infrastructures play a crucial part in exploiting vulnerabilities, their behaviors are often treated as an auxiliary when defining and monitoring a botnet family.
% This sample-centered convention confines 
% Conventional sample-centered methodologies confines botnet virology to a client-based perspective yet may distort gathered threat intelligence about relationships of botnets.
While dissecting malware samples and conducting the dynamic analysis can provide solid evidence to depict the genealogy of botnet families, conventional sample-centered methodologies pay less attention to their infrastructure components and confine botnet virology to a client-based perspective.
The server-side knowledge about their cloud-based loaders is incomplete due to the absence of samples, which makes existing CTIs suffer from a distortion in understanding the relationship of their compromising toolkits.
% =======================================
By investigating bot loaders' compromising toolkits, this work seeks to complement the deficiency of botnet virology from the server-side perspective.
We propose a semantic-aware methodology to understand the command components from infection requests, then describe their ``homology" to discuss shared ones across different loader instances.
Based on this knowledge, we categorized loaders into several families from a pure server-side perspective and compare our conclusions with existing virus scanners.
We further discussed the consistency and inconsistency between our conclusion and those derived from conventional methods.
As the released code of Mirai keeps spawning new generations of botnets both on the client and the server side, this paper uncovers the diversity of their compromising toolkits and infrastructures and sheds light on a new perspective on finding covert relationships among cybercrimes.

\endinput 

==> parts/v2-journal/01-intro-v2.tex <==
% !TeX root = ..\main.tex
Accompanying the growth of the IoT market, botnets targeting IoT devices have become a major threat to cyber security.
Early in 2016, The emerging Mirai botnet drew attention from the cybersecurity community\cite{malwaremustdie!MMD00562016LinuxMirai2016}.
It launched a 1.1Tbps DDoS attack using 148,000 IoT devices, breaking the record and making it the most notorious botnet clan in the following years.
As the released code of the original Mirai\cite{anna-senpaiFREEWorldLargest2016} created an persistently active ecology of botnet, cybersecurity community strived to enable an taxonomic view to better understand emerging variants and systematically describe their similarities.
Multiple \textit{families} were defined by general taxonomy studies\cite{antonakakisUnderstandingMiraiBotnet2017,herwigMeasurementAnalysisHajime2019,griffioenExaminingMiraiBattle2020} while \textit{variants} are identified and categorized mostly by dissecting collected malware samples\cite{cozziTangledGenealogyIoT2020,downingDeepReflectDiscoveringMalicious2021,wangEvolutionaryStudyIoT2021}.

However, while sample-centered analyses could depict lineage or genealogy among malware families and variants, some server-side components are still overlooked in the context of Mirai-like botnets. 
Unlike conventional worms infecting new victims independently, Mirai introduced a decoupled design to infection toolkits and migrated these functions to a self-contained \emph{loader server}.
This design simplified infection module in bot clients to only scan and report exploitable victims to the loader server, which successfully makes bots less resource-consuming.

The IoT-friendly improvement split a botnet system into two disjoint parts, which makes upgrading intrusion toolkits extremely convenient, but also brought much concern to understanding botnets as an integrated system.
When discussing the variation and evolution of infection toolkits, the asynchronized development of bot clients and loaders makes it inappropriate to simply take knowledge of families derived from samples.
Moreover, as these cloud-based loaders are seldom distributed like bot clients, the sample-based lineage inference also infeasible due to the limitation of honeypots.

In this paper, we go deep into the most widely adopted infection toolkit, the telnet loader, to provide a server-side view of botnets' variation and evolution with absent loader samples.
To address the absence of captured samples, we treat interaction logs from telnet honeypots as objective representations of intrusion toolkits.
We leverage a semantic-aware method to examine their intrusion commands, then further discover their similarities and variations under the conventional family-variant epistemology.
Our work provides a behavior-based categorization of bot loaders and proposes a new homology view on bot loaders, helping researchers obtain deeper knowledge about IoT botnets.
The main contributions of our work are summarized as follows:

\begin{itemize}
  \item
    Our work complements the server-side perspective by depicting the active variation of telnet bot loaders.
    While it is commonly overlooked due to the absence of samples, we study intrusion logs from honeypots using a semantic-aware method to describe loaders' functions and systematically compare observed instances.
  \item
    We apply the conventional family-variant epistemology to the server-side view and make a taxonomic study about observed bot loaders.
    Based on agglomerative clustering, we define 8 families to discuss their shared patterns and genealogy of intrusion toolkits.
  \item % 揭露botloader也产生了变种与变化，需要单独讨论。
    As previous studies have disclosed the evolution of Mirai bots, our conclusion reveals the concurrent evolution of loaders, which demonstrates the importance of the server-side prospect in botnet provenance attribution.
\end{itemize}

\endinput

==> tables/geoip.tex <==
% !TeX root = ..\main.tex
\begin{table}[htbp]
    \centering
    \caption{Distribution of loader hosts in autonomy systems}
    \begin{tabular}{cccc}
      \hline
      \textbf{Country} & \textbf{Name}                                     & \textbf{Hosts} & \textbf{Logs} \\ \hline
      China            & CHINA UNICOM China169 Backbone                    & 184            & 2145              \\
      India            & Hathway IP Over Cable Internet                    & 29             & 361               \\
      Russia           & MTS PJSC                                          & 29             & 360               \\
      China            & Chinanet                                          & 28             & 286               \\
      India            & National Internet Backbone                        & 20             & 243               \\
      \hline
      \textit{Others}  & \textit{}                                         & \textit{237}   & \textit{1454}     \\
      \hline
    \end{tabular}
    \label{table_as_dist}
\end{table}
  
